Learning Two-Stream CNN for Multi-Modal Age-related Macular Degeneration Categorization

This paper tackles automated categorization of Age-related Macular Degeneration (AMD), a common macular disease among people over 50. Previous research efforts mainly focus on AMD categorization with a single-modal input, let it be a color fundus photograph (CFP) or an OCT B-scan image. By contrast, we consider AMD categorization given a multi-modal input, a direction that is clinically meaningful yet mostly unexplored. Contrary to the prior art that takes a traditional approach of feature extraction plus classifier training that cannot be jointly optimized, we opt for end-to-end multi-modal Convolutional Neural Networks (MM-CNN). Our MM-CNN is instantiated by a two-stream CNN, with spatially-invariant fusion to combine information from the CFP and OCT streams. In order to visually interpret the contribution of the individual modalities to the final prediction, we extend the class activation mapping (CAM) technique to the multi-modal scenario. For effective training of MM-CNN, we develop two data augmentation methods. One is GAN-based CFP/OCT image synthesis, with our novel use of CAMs as conditional input of a high-resolution image-to-image translation GAN. The other method is Loose Pairing, which pairs a CFP image and an OCT image on the basis of their classes instead of eye identities. Experiments on a clinical dataset consisting of 1,094 CFP images and 1,289 OCT images acquired from 1,093 distinct eyes show that the proposed solution obtains better F1 and Accuracy than multiple baselines for multi-modal AMD categorization. Code and data are available at https://github.com/li-xirong/mmc-amd.

==> backup-related-da.tex <==
The achievement of a CNN model highly depends on sufficiently large datasets. However, in many realistic scenes, we have to achieve goals with limited datasets, particularly in medical image domain. Data augmentation solves the problem to some extend by generating variants of original training data. 

%As in multi-modal domain, input is organized in pair, we investigate the data augmentation approaches at both image-level and pair-level.

%\paragraph{Image-level data augmentation}
Conventional data augmentation applies various transformation on training data \cite{krizhevsky2012imagenet}, including random crop, rotation, flip, \etc Although this strategy is so vital that it is widely used in many visual computing researches, the diversity of such variants is limited by the finite transformations. By contrast, GAN based data augmentation creates adversarial samples with richer varieties \cite{antoniou2017data}.

GAN is a generative model framework to build mapping function from noisy data to the distribution of a certain dataset. In order to control on modes of the generated data, conditional GAN \cite{mirza2014conditional} adds conditioned label on input, such as class label or segmentation map. GANs are widely used in the medical image domain \cite{yi2019generative}, including reconstruction \cite{yang2017dagan,zhang2018multi}, cross modality synthesis \cite{hiasa2018cross,yu20183d} and data augmentation \cite{frid2018gan,shin2018medical,xing2019adversarial}. As for ophthalmic image analysis, such framework achieves to process both color fundus \cite{costa2017end,lahiri2017generative,mahapatra2017retinal} and OCT \cite{schlegl2017unsupervised}. 
 
 %% GANs achieve to generated fundus from a vessel image or segment vessel from a given fundus \cite{costa2017end,lahiri2017generative,mahapatra2017retinal}. Schlegl \etal propose an unsupervised method for anomaly detection on OCT image via a GAN to recognize abnormalities \cite{schlegl2017unsupervised}.

GAN-based data augmentation appear in various medical images computing tasks \cite{frid2018gan,shin2018medical,xing2019adversarial}. These work leverage conditional GANs with various conditioned labels to guide the class and the image characters of the synthesis.
\paragraph{Vector-to-image synthesis} 
Onehot vector of the class is the simplest conditioned label. Such presentation is available as long as the data is categorized. Frid \etal \cite{frid2018gan} train an ACGAN \cite{odena2017conditional} where the lesion class onehot is applied as conditioned label to generate liver cysts lesions. These adversarial samples improve the lesion classification task.

\paragraph{Image-to-image synthesis}
In order to control more specific details in the synthetic image, image-to-image translation GAN employs spatial relevant maps, \ie segmentation map, edge map, \etc, as conditioned labels, to offer detailed condition at pixel-level \cite{isola2017image,wang2018high}. Image-to-image translation is used to generate abnormalities or biological structure in medical image synthesis. Shin \etal \cite{shin2018medical} integrate different segmentation labels, tissue segmentation and tumor segmentation, from two independent brain-MRI dataset by an MRI-to-label GAN (pix2pixGAN \cite{isola2017image}), and then synthesize MRIs with tumor by a label-to-MRI GAN (pix2pixGAN). The adversarial MRIs make progress in learning tumor segmentation. Xing \etal \cite{xing2019adversarial} aim to insert real lesions into synthetic images of chest X-ray. They condition a pix2pixGAN by a mask of abnormal images where only the bounding boxes of lesions are maintained and other regions are set to zero. The generated samples benefit their lesion detection task.

Note that vector-to-image GAN only asks class label and gives rough synthesis while image-to-image GAN generates details but requiring manual annotation maps which are usually unavailable. In this paper, we aims to synthesize \textit{approximate} abnormalities with absence of any manual-annotated label map. We used CAM to direct the generating process, because such map contains the approximate size, location and severity information (activation value) of abnormalities. Meanwhile, it's auto-generated and non-manual. We regard CAM-to-image as an image-to-image translation task and follow the model design of pix2pixHD \cite{wang2018high}. 

%% \paragraph{Pair-level data augmentation} 
%% Considering that the multi-modal input is formed in pair, it's a nature thought to augment data at the pair level. However, to the best of our knowledge, the direction is less explored. Luo \etal \cite{luo2019gan} use GAN technique to directly generate concatenated feature from different modality for multi-modal emotion recognition. Their setting increases data varieties at multi-modal level. In our work, we propose an image-pair sampling approach that pairs fundus and OCT based on the same label rather than the same eye. Such a simple strategy shows large effect.



==> big-results-tab.tex <==
\begin{table}[tbh!]
    \normalsize
    \renewcommand\arraystretch{1.2}
    \centering
    \caption{\textbf{The performance on all Partitions}.}
    \label{tab:partitions}
    \scalebox{0.64}{
    \begin{tabular}{@{}|c|l | r | r | r | r | r|r |@{}}
    \hline
    \multirow{2}{*}{\textbf{Partition}} &\multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c|}{\textbf{F1-score}}  & \multirow{2}{*}{\textbf{Accuracy}}\\
    \cline{3-7}
    & & \textit{normal} & \textit{dryAMD}  & \textit{PCV}  & \textit{wetAMD} & \textit{Overall} & \\

    \hline\hline
    \multirow{4}{*}{\textbf{A}}
    & \revise{CFP-CNN} & \textbf{1.000} & 0.798 & 0.638 & 0.661 & 0.774 & 0.717 \\
    \cline{2-8}
    & OCT-CNN	   & \textbf{1.000} & \textbf{0.934} & 0.810 & 0.801 & 0.886 & 0.818 \\
    \cline{2-8} 
    & MM-CNN 		 & \textbf{1.000} & 0.847 & 0.841 & 0.801 & 0.872 & 0.804 \\
    \cline{2-8}
    & MM-CNN-\textit{da}  & \textbf{1.000} & 0.929 & \textbf{0.864} & \textbf{0.864} & \textbf{0.914} & \textbf{0.863} \\

    \hline\hline
    \multirow{4}{*}{\textbf{B}}
    & \revise{CFP-CNN} & 0.992 & 0.504 & 0.619 & 0.675 & 0.697 & 0.625 \\
    \cline{2-8}
    & OCT-CNN	   & \textbf{1.000} & 0.826 & 0.747 & 0.735 & 0.827 & 0.736 \\
    \cline{2-8} 
    & MM-CNN 		 & \textbf{1.000} & 0.712 & 0.678 & 0.726 & 0.779 & 0.700 \\
    \cline{2-8}
    & MM-CNN-\textit{da}  & 0.999 & \textbf{0.965} & \textbf{0.762} & \textbf{0.819} & \textbf{0.886} & \textbf{0.824} \\

    \hline\hline
    \multirow{4}{*}{\textbf{C}}
    & \revise{CFP-CNN} & \textbf{1.000} & 0.597 & 0.583 & 0.525 & 0.676 & 0.592 \\
    \cline{2-8}
    & OCT-CNN	   & \textbf{1.000} & \textbf{0.882} & 0.756 & 0.738 & 0.844 & 0.764 \\
    \cline{2-8} 
    & MM-CNN 		 & \textbf{1.000} & 0.708 & 0.621 & 0.626 & 0.739 & 0.622 \\
    \cline{2-8}
    & MM-CNN-\textit{da}  & \textbf{1.000} & 0.877 & \textbf{0.800} & \textbf{0.739} & \textbf{0.854} & \textbf{0.778} \\

    \hline\hline
    \multirow{4}{*}{\textbf{D}}
    & \revise{CFP-CNN} & \textbf{1.000} & 0.523 & 0.818 & 0.697 & 0.760 & 0.692 \\
    \cline{2-8}
    & OCT-CNN	   & \textbf{1.000} & \textbf{0.936} & 0.874 & 0.594 & 0.851 & 0.813 \\
    \cline{2-8} 
    & MM-CNN 		 & \textbf{1.000} & 0.856 & 0.827 & 0.546 & 0.807 & 0.742 \\
    \cline{2-8}
    & MM-CNN-\textit{da}  & \textbf{1.000} & 0.935 & \textbf{0.889} & \textbf{0.718} & \textbf{0.885} & \textbf{0.833} \\

    \hline\hline
    \multirow{4}{*}{\textbf{E}}
    & \revise{CFP-CNN} & \textbf{1.000} & 0.755 & 0.754 & \textbf{0.747} & 0.814 & 0.750 \\
    \cline{2-8}
    & OCT-CNN	   & 0.999 & 0.891 & 0.777 & 0.667 & 0.833 & 0.757 \\
    \cline{2-8} 
    & MM-CNN 		 & \textbf{1.000} & 0.714 & 0.779 & 0.717 & 0.803 & 0.704 \\
    \cline{2-8}
    & MM-CNN-\textit{da}  & 0.996 & \textbf{0.926} & \textbf{0.802} & 0.726 & \textbf{0.862} & \textbf{0.794} \\
    
    \hline
    \end{tabular}
    }
    \end{table}
    

==> data_tab_part.tex <==
\begin{table}[tbh!]
\renewcommand{\arraystretch}{1.2}
\centering
\caption{\textbf{Data split of PartitionB-E}. \ws{In each partition, training set, validation set, and test set are divided based on eyes. In parentheses are number of eyes per class in each set.} As the number of OCT images varies per eye, OCT images of the four classes are more unbalanced. }\label{tab:data_part}
\scalebox{0.77}{
\begin{tabular}{|c| l| r|r | r|r | r|r |}
\hline
   
\multirow{2}{*}{\textbf{Partition}} & \multirow{2}{*}{\textbf{Class}} & \multicolumn{2}{c|}{\textbf{Training set}} & \multicolumn{2}{c|}{\textbf{Validation set}}  & \multicolumn{2}{c|}{\textbf{Test set}}  \\
\cline{3-8}
& & \textit{Fundus} 	& \textit{OCT} 	& \textit{Fundus} 	& \textit{OCT}	& \textit{Fundus} 	&  \textit{OCT} \\
\hline
\hline

\multirow{4}{*}{\textbf{B}}  
& \textit{normal} 	& 155 (155) 		& 156 (155)		& 20 (20) 			& 20 (20)  	& 20 (20)			& 20 (20) \\
\cline{2-8}
& \textit{dryAMD} 	& 67 (~67) 		& 36 (~22) 		& 20 (20)			&  33 (20) 	& 20 (20)			& 37 (20) \\
\cline{2-8}
& \textit{PCV} 	& 261 (261) & 295 (157) & 20 (20) & 43 (20)  & 20 (20)	& 42 (20) \\
\cline{2-8}
& \textit{wetAMD} 	& 456 (456) 		& 533 (327) 		& 20 (20)			&  34 (20) 	& 20 (20)			& 41 (20) \\
\hline
\hline

\multirow{4}{*}{\textbf{C}}  
& \textit{normal} 	& 155 (155) 		& 156 (155)		& 20 (20) 			& 20 (20)  	& 20 (20)			& 20 (20) \\
\cline{2-8}
& \textit{dryAMD} 	& 67 (~67) 		& 41 (~22) 		& 20 (20)			& 31 (20)  	& 20 (20)			& 34 (20) \\
\cline{2-8}
& \textit{PCV} 	& 261 (261) & 303 (157) & 20 (20) & 39 (20)  & 20 (20)	& 38 (20) \\
\cline{2-8}
& \textit{wetAMD} 	& 456 (456) 		& 547 (327) 		& 20 (20)			& 33 (20)  	& 20 (20)			& 28 (20) \\
\hline
\hline

\multirow{4}{*}{\textbf{D}}  
& \textit{normal} 	& 155 (155) 		& 156 (155)		& 20 (20) 			& 20 (20)  	& 20 (20)			& 20 (20) \\
\cline{2-8}
& \textit{dryAMD} 	& 67 (~67) 		& 34 (~22) 		& 20 (20)			& 37 (20)  	& 20 (20)			& 35 (20) \\
\cline{2-8}
& \textit{PCV} 	& 261 (261) & 300 (157) & 20 (20) & 41 (20)  & 20 (20)	& 39 (20) \\
\cline{2-8}
& \textit{wetAMD} 	& 456 (456) 		& 537 (327) 		& 20 (20)			& 37 (20)  	& 20 (20)			& 34 (20) \\
\hline
\hline

\multirow{4}{*}{\textbf{E}}  
& \textit{normal} 	& 155 (155) 		& 156 (155)		& 20 (20) 			& 20 (20)  	& 20 (20)			& 20 (20) \\
\cline{2-8}
& \textit{dryAMD} 	& 67 (~67) 		& 34 (~22) 		& 20 (20)			& 32 (20)  	& 20 (20)			& 40 (20) \\
\cline{2-8}
& \textit{PCV} 	& 261 (261) & 305 (157) & 20 (20) & 33 (20)  & 20 (20)	& 42 (20) \\
\cline{2-8}
& \textit{wetAMD} 	& 456 (456) 		& 537 (327) 		& 20 (20)			& 40 (20)  	& 20 (20)			& 31 (20) \\
\hline
\end{tabular}
}
\end{table}

